Laying the Foundation First? Investigating the Generalization from Atomic Skills to Complex Reasoning Tasks

Current language models have demonstrated their capability to develop basic reasoning, but struggle in more complicated reasoning tasks that require a combination of atomic skills, such as math word problem requiring skills like arithmetic and unit conversion. Previous methods either do not improve the inherent atomic skills of models or not attempt to generalize the atomic skills to complex reasoning tasks. In this paper, we first propose a probing framework to investigate whether the atomic skill can spontaneously generalize to complex reasoning tasks. Then, we introduce a hierarchical curriculum learning training strategy to achieve better skill generalization. In our experiments, we find that atomic skills can not spontaneously generalize to compositional tasks. By leveraging hierarchical curriculum learning, we successfully induce generalization, significantly improve the performance of open-source LMs on complex reasoning tasks. Promisingly, the skill generalization exhibit effective in cross-dataset and cross-domain scenarios. Complex reasoning can also help enhance atomic skills. Our findings offer valuable guidance for designing better training strategies for complex reasoning tasks.

==> tables/mwp_example.tex <==

\begin{table}[t]
\footnotesize


  \centering
  \renewcommand{\arraystretch}{1.0}

\resizebox{0.48\textwidth}{80mm}{
    \begin{tabularx}{\linewidth}{X}
    \toprule
    \rowcolor[gray]{0.95}\multicolumn{1}{c}{\textbf{I: Math Word Problem (Compositional Task)}} \\
    \midrule
    \textbf{Question}: Andy walks 50 meters from his house to school. After school, he comes back to the house and goes to the market. If he walks 140 meters in total, how many kilometer is the distance between the house and the market? \\
    \textbf{Answer}: He walks 50m from home to school and walks 50m again from school to house, so he walks \textcolor{red}{50 + 50 = 100} meters. If the total distance is 140m, the distance between the house and the market is 140m - 100m = 40 meters. \textcolor{blue}{40 meters is equal to 0.04 kilometer}. So the answer is 0.04 kilometer.

    \midrule
    
    \rowcolor[gray]{0.95}\multicolumn{1}{c}{\textbf{II: Arithmetic Data (Prerequisite Task)}} \\
    \midrule
    \textbf{AddSub}: 123 + 5315 = 4538 </s> 23.45 + 124 = 147.45 ...\\
    \textbf{S-Mul:} 1313 * 0.2 = 262.6 </s> 144 * 50 = 7200 ...  \\
    \textbf{C-Mul:} 13 * 31.3 = 13 * 30 + 13 * 1 + 13 * 0.1 \\
                              = 390 + 13 + 1.3 \\
                              = 403 + 1.3 \\
                              = 404.3 \\
    \textbf{S-Div:} 

    \hdashline


    \textcolor[rgb]{0.5,0.5,0.5}{/* \textit{Task E: Dimension Prediction} */}\\
    \textbf{Question}:
    Please predict the corresponding SI base unit for the [MASK] part missing in the following sentence. \\
    \textbf{Sentence}: The Tawuza hydroelectric power station has an annual output of [MASK], providing reliable power support for local industries and residents.\\
    Options: (A)m2·kg/mol·s2 (B)m2·kg/A·s2 (C)m3·kg/s2 (D)m2·kg/s2 \\
    \textbf{Answer:} (D) \\

    \midrule
    \rowcolor[gray]{0.95}\multicolumn{1}{c}{\textbf{III: Scale Perception}} \\
    \midrule

    \textcolor[rgb]{0.5,0.5,0.5}{/* \textit{Task F: Unit Conversion} */}\\
    \textbf{Question}:In terms of the physical quantity Density, how many milligrams per decilitre is equal to 1 kg/m3?\\
    Options: (A)10.0 (B)1000.0 (C)100.0 (D)200.0\\
    \textbf{Answer:} (C) \\

    \hdashline
    \textcolor[rgb]{0.5,0.5,0.5}{/* \textit{Task G: Maximal Magnitude Retrieval} */}\\
    \textbf{Question}:Which of the following four physical quantities is the largest one? \\
    Options: (A)1e16 cm (B)1 light year (C)507.5613 Mile (D)1e20 fermi\\
    \textbf{Answer:} (A) \\

\caption{caption.}
\label{tab:dimperc_example}
     
    \bottomrule
    \end{tabularx}
}
  
\end{table}



